Receler: Reliable Concept Erasing of Text-to-Image Diffusion Models via Lightweight Erasers

Concept erasure in text-to-image diffusion models aims to disable pre-trained diffusion models from generating images related to a target concept. To perform reliable concept erasure, the properties of robustness and locality are desirable. The former refrains the model from producing images associated with the target concept for any paraphrased or learned prompts, while the latter preserves its ability in generating images with non-target concepts. In this paper, we propose Reliable Concept Erasing via Lightweight Erasers (Receler). It learns a lightweight Eraser to perform concept erasing while satisfying the above desirable properties through the proposed concept-localized regularization and adversarial prompt learning scheme. Experiments with various concepts verify the superiority of Receler over previous methods.

==> Figures/multi_class.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/images/multi_class.pdf}
  \caption{
  \textbf{Visualization examples of compositional concept erasure.}
  Instead of training an eraser for multiple concepts, we can combine existing erasers for multi-concept erasure, each corresponding to an unlearned concept.
  }
  \label{fig:multi_class}
\end{wrapfigure}

